BabelCoder: Agentic Code Translation with Specification Alignment

As software systems evolve, developers increasingly work across multiple programming languages and often face the need to migrate code from one language to another. While automatic code translation offers a promising solution, it has long remained a challenging task. Recent advancements in Large Language Models (LLMs) have shown potential for this task, yet existing approaches remain limited in accuracy and fail to effectively leverage contextual and structural cues within the code. Prior work has explored translation and repair mechanisms, but lacks a structured, agentic framework where multiple specialized agents collaboratively improve translation quality. In this work, we introduce BabelCoder, an agentic framework that performs code translation by decomposing the task into specialized agents for translation, testing, and refinement, each responsible for a specific aspect such as generating code, validating correctness, or repairing errors. We evaluate BabelCoder on four benchmark datasets and compare it against four state-of-the-art baselines. BabelCoder outperforms existing methods by 0.5%-13.5% in 94% of cases, achieving an average accuracy of 94.16%.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> limitation.tex <==
\section{\color{red}Limitation}
{\color{red} R1.6 Although the Test Agent is claimed to support multiple languages, the TransCoder dataset focuses only on the Python-to-Java translation direction, while CodeNet includes 20 language pairs. The paper attributes this limitation to the availability of a unit test converter, yet this component is not formally defined in the system design. The authors are encouraged to clarify why support for additional language pairs is constrained by a component that is not explicitly included in the Test Agent.}

==> multiagent_results.tex <==
\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1.2}
\caption{Translation accuracy across various source and target languages.}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Dataset} & \textbf{Source} & \textbf{Target} & \textbf{Accuracy on} & \textbf{Accuracy on} & \textbf{LIT \& UniTrans} \\

&  &  & \textbf{generated tests (\%)} & \textbf{evaluation tests (\%)} & \textbf{Results (\%)} \\
\hline
\multirow{8}{*}{avatar} & \multirow{4}{*}{Java}     & C & 96.67 & 95.83 & 82.33 \\
                        &                           & C++ & 96.67 & 98.75 & 91.97 \\
                        &                           & Go & 80.42 & 87.08 & 80.72 \\
                        &                           & Python & 88.75 & 92.5 & 85.94 \\ \cline{3-6}
                        & \multirow{4}{*}{Python}   & C & 82.91 & 75.73 & 62 \\
                        &                           & C++ & 86.25 & 83.26 & 70 \\
                        &                           & Go & 80.83 & 80.33 & 63.6 \\
                        &                           & Java & 88.33 & 87.87 & 76.4 \\
\hline

\multirow{20}{*}{codenet}   & \multirow{4}{*}{C}        & C++ & 94.5 & 99 & 98.5 \\
                            &                           & Go & 79.5 & 87.5 & 93 \\
                            &                           & Java & 91.5 & 98 & 96.5 \\
                            &                           & Python & 84.5 & 93 & 89.5 \\ \cline{3-6}
                            & \multirow{4}{*}{C++}      & C & 95 & 98 & 97 \\
                            &                           & Go & 85.5 & 94 & 94.5 \\
                            &                           & Java & 93.5 & 98 & 97.5 \\
                            &                           & Python & 93 & 94 & 89.5 \\ \cline{3-6}
                            & \multirow{4}{*}{Go}       & C & 95 & 97.5 & 96 \\
                            &                           & C++ & 98 & 98.5 & 97 \\
                            &                           & Java & 95.5 & 99 & 95.5 \\
                            &                           & Python & 94 & 96.5 & 90.5 \\ \cline{3-6}
                            & \multirow{4}{*}{Java}     & C & 92.5 & 97.5 & 93.5 \\
                            &                           & C++ & 92 & 98 & 96 \\
                            &                           & Go & 77 & 87.5 & 91.5 \\
                            &                           & Python & 88.5 & 94 & 91.5 \\ \cline{3-6}
                            & \multirow{4}{*}{Python}   & C & 94.5 & 98 & 94.5 \\
                            &                           & C++ & 97 & 99.5 & 96 \\
                            &                           & Go & 90 & 94 & 88 \\
                            &                           & Java & 96 & 99 & 96.5 \\
\hline
evalplus & Python & Java & 92.68 & 90.85 & 84.76 \\
\hline
transCoder test & Python & Java & 92.24 & - & 87.07 (UniTrans) \\
\hline
\end{tabular}
\label{tab:translation_accuracy}
\end{table*}


==> results.tex <==
\section{Results}
\label{results}

% \noindent In this section, we revisit the RQs and provide answers based on our findings.

\subsection*{RQ1: \RQOne}
\pa{Motivation.} Existing works evaluate code translation using different benchmarks, CodeNet and Avatar using standard input/output, and TransCoder and EvalPlus using functional correctness. To enable a comprehensive comparison, RQ1 investigates whether our agent-based framework can consistently outperform these approaches across all four benchmarks.

\pa{Method.} To answer this question, we run \tool{} end-to-end on the datasets in Section~\ref{datasets}. Then, we compare the results against the baselines outlined in Section~\ref{baselines}. For Avatar and CodeNet, we use the same samples as LIT~\citep{pan2024lost}, ensuring a fair comparison. For EvalPlus, we conduct experiments on the full dataset. Since UniTrans~\citep{yang2024exploring} uses GPT-3.5 on the TransCoder~\citep{lachaux2020unsupervised} dataset, we also use GPT-3.5 in our experiments for fair comparison. Similarly, as TransAgent uses gpt-4 on the TransCoder dataset, we used the same model in our experiments.

\input{multiagent_results_with_baselines}

\pa{Result.} The outcomes are summarized in Table~\ref{tab:translation_accuracy}. For \tool, we reported the CA for both provided test cases for comparison with LIT and generated test cases for comparison with UniTrans and TransAgent.
As seen in the table, our framework consistently achieves significantly better performance than the three baselines by 0.5\% to 13.5\% across all language pairs using the same setting, except for three cases: C++-Go, C-Go, and Java-Go in the CodeNet dataset. For C++-Go, \tool{} achieves equivalent performance to the baseline, i.e., LIT.
For C-Go and Java-Go in CodeNet, LIT outperforms \tool{} by 5.5\% and 4\% respectively. 
We believe this discrepancy stems from the nature of the CodeNet evaluation suite, which provides only a single test case per sample. This tends to produce more conservative or generic translations, which may happen to pass the single evaluation test more often, even if they are less correct overall. In contrast, our framework relies on multiple gpt-4-generated tests to guide the translation and repair process; the limited evaluation coverage (single tests) may not fully reflect the improvements made by our method.

Overall, results using the evaluation tests are consistently better than those using gpt-4-generated tests, which indicates that gpt-4 is capable of generating diverse and more challenging test cases that facilitate effective program repair.

As described in Section~\ref{intertrans-baseline}, we compare \tool{} with InterTrans using the same 31 samples. InterTrans invokes the model up to 313 times per translation and leverages the target function’s header to guide generation. In contrast, \tool{} achieves the same accuracy on these samples without those, demonstrating greater efficiency and generality.
\input{sonarqube}

\subsection*{RQ2. \RQTwo}
\label{rq2}
\pa{Motivation.} During code translation between significantly different programming languages, software quality, especially security, becomes a major concern. This research question investigates the extent to which translation affects code quality, focusing specifically on security-related issues and general software defects before and after translation. 

\pa{Method.} To address this question, we analyze both the original source code and the corresponding translated code from our four datasets using \textit{SonarQube}~\citep{sonarqube}. SonarQube is chosen for its ability to automatically detect a wide range of software quality issues, including security vulnerabilities (e.g., injection flaws, access control) and maintainability issues (e.g., code smells, duplications). Our analysis concentrates on two key categories reported by \textit{SonarQube}: blocker and critical issues, which typically include severe bugs and security vulnerabilities. Besides, we consider any flagged security hotspots or direct vulnerabilities identified in the code. To normalize the comparison across files of varying size, we report the number of issues per 1,000 lines of non-commented source code (NLOC).

\pa{Result.} Table~\ref{tab:translation_issues} presents the identified issues and associated security impacts in both the source and translated code across all selected datasets. The results show that when translating from other languages to C, the number of issues consistently increases by 18.35 to 35.86 per 1000 NLOC. A similar trend is observed for security impacts, which also rise by 4.9 to 10.82 per 1000 NLOC when translated into C. One possible explanation for this behavior is that C lacks many high-level abstractions and safety features (e.g., memory management, type safety) available in other languages, making it more prone to translation-related bugs and vulnerabilities.
Interestingly, when translating from C++ to C, the number of issues does not increase. In contrast, translating from C to C++ produces 18.66 more issues per 1000 NLOC. This observation may offer a useful insight: to reduce translation-induced issues, it could be beneficial to use an intermediate language such as C++. For example, translating from another language to C++ and then to C might help limit the number of introduced issues. A deeper investigation into this approach is beyond the scope of this study and is left for future work.

\subsection*{RQ3. \RQThree}
\pa{Motivation.} As the Refinement Agent is one of the contributions of this study, we are interested in knowing how different parts (Initial Translation and Fixation, \NLSpecS Augmentation, \NLSpecS Validation, and Bug Scope Estimation) of this Refinement Agent perform.

\pa{Method.} To address this research question, we perform an ablation study by disabling and subsequently enabling the \NLSpecS augmentation, validation (Sec \ref{nl-agumentation} \& \ref{nl-validation}), and Bug Scope Estimation (Sec \ref{bug-scope-estimation}) module in our approach. At each of these stages, we generate translations and evaluate them using the evaluation test cases provided with the benchmark datasets.

In the first stage, translations are generated solely based on the source code and optionally refined by the Refinement Agent, but without involving \NLSpecS generation, validation, or Bug Scope Estimation. In the second stage, translations are generated using \NLSpecS, with state tracking enabled. These translations are then refined using Spectrum-Based Fault Localization (SBFL), and LLM-based bug-fix modules. At the later stages, we enable the \NLSpecS verification, Bug-Scope Estimation module of the Refinement Agent.

This ablation study evaluates the functional correctness of the translated code using the test suites included in the datasets. Consequently, the study is conducted on the first three benchmark datasets described in Section~\ref{datasets}. The fourth dataset \citep{lachaux2020unsupervised, yang2024exploring} is excluded from this analysis due to missing evaluation test cases.

\input{ablation_study_result}

\pa{Result.} As reported in Table~\ref{tab:ablation_study}, an average of 87.28\% of translations passed the evaluation in the first stage, where \NLSpecS generation, validation, and bug scope estimation modules were disabled. At the second stage, we augmented \NLSpecS and, thus, we have gained 92.85\% computational accuracy with a 6.39\% increment over the previous stage. After adding \NLSpecS validation, the computational accuracy reached 93.72\%, and with Bug Scope estimation, the accuracy reached 94.16\%.

{\color{blue}
\subsection*{RQ3. \RQThreeNew}

\begin{table}[t]
\centering
\caption{Sequential ablation study on EvalPlus (Python$\rightarrow$Java, GPT-4o, $N=164$).
Each row cumulatively adds one component over the previous.
CA\textsubscript{gen} is evaluated on generated test cases;
CA\textsubscript{eval} is evaluated on ground-truth tests.}
\label{tab:ablation}
\begin{tabular}{clcc}
\toprule
\textbf{Config} & \textbf{Component Added}
  & \textbf{CA\textsubscript{gen} (\%)}
  & \textbf{CA\textsubscript{eval} (\%)} \\
\midrule
C6 & Translate + compile fix only         & --    & 79.88 \\
C1 & + Test-driven repair                 & 84.76 & 85.37 \\
C3 & + NLSpec guidance (no source)        & 89.63 & 88.41 \\
C2 & + Alignment validator                & 91.46 & 89.63 \\
C4 & + Source code in prompt              & 92.68 & 90.24 \\
C7 & + Full pipeline minus BugScope       & 93.29 & 90.24 \\
\midrule
C5 & + BugScope classifier (BabelCoder)   & \textbf{93.29} & \textbf{91.46} \\
\bottomrule
\end{tabular}
\end{table}


\begin{figure}[]
    \centering
    \includegraphics[
        width=\textwidth,
        height=0.92\textheight,
        keepaspectratio
    ]{ablation_figure.pdf}
    \caption{Ablation study results showing the contribution of individual 
             and sequential model components. Each configuration removes or 
             adds one component at a time to isolate its effect on generation 
             (Gen) and evaluation (Eval) performance across the test set.}
    \label{fig:ablation}
\end{figure}

{\color{blue}
\subsection*{RQ4. \RQFour}

\pa{Motivation.} \tool{} operates at a temperature of 0.8, which introduces non-determinism across the multi-agent pipeline. A reviewer raised the concern that reporting a single run may not sufficiently reflect the robustness of the system. Traditional pass@$k$ metrics~\citep{chen2021evaluating} are designed for single-function generation scenarios, where $k$ independent samples are drawn from one LLM call. However, \tool{} is a stateful, sequential pipeline consisting of approximately ten chained LLM calls per instance (Translation Agent $\rightarrow$ Refinement Agent $\rightarrow$ Test Agent $\rightarrow$ Bug Localization $\rightarrow$ Repair Agent), where each agent conditions on the output of the previous one. Sampling independently at the token level is therefore architecturally inappropriate~\citep{yao2024tau, shinn2023reflexion, islam2024mapCoder}; a meaningful robustness measure must account for variance at the pipeline level. This RQ investigates whether \tool{} achieves stable and consistent performance across multiple independent end-to-end executions on the EvalPlus benchmark.

\pa{Method.} To address this question, we execute the full \tool{} pipeline five independent times on the EvalPlus dataset (164 Python-source instances), keeping all hyperparameters fixed (temperature = 0.8, GPT-4o). Each run constitutes a complete, independent pipeline execution with fresh intermediate states. We report the Computational Accuracy (CA) for each individual run, the mean CA with standard deviation ($\mu \pm \sigma$) across the five runs, and pass@5. 

Following~\citet{chen2021evaluating}, we adapt the pass@$k$ estimator to the pipeline level: for each problem instance $i$, let $c_i$ be the number of runs (out of $n = 5$) that produce a correct translation. Then:
\begin{equation}
    \text{pass@}k = \mathbb{E}_{i}\!\left[1 - \frac{\binom{n - c_i}{k}}{\binom{n}{k}}\right]
    \label{eq:passk}
\end{equation}
where the expectation is taken over all 164 problem instances. This formulation captures the probability that at least one of $k$ independent pipeline runs yields a correct translation, and is reported for $k = 5$.

\begin{table}[h]
\centering
\caption{{\color{red}DUMMY TABLE: }Computational Accuracy (\%) of \tool{} across 5 independent runs on EvalPlus (Python source, 164 instances, GPT-4o, temperature = 0.8). $\mu \pm \sigma$ = mean $\pm$ standard deviation; pass@5 computed per Eq.~\ref{eq:passk}.}
\label{tab:rq4_stability}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|ccccc|cc}
\toprule
\textbf{Lang. Pair} & \textbf{Run 1} & \textbf{Run 2} & \textbf{Run 3} & \textbf{Run 4} & \textbf{Run 5} & $\boldsymbol{\mu \pm \sigma}$ & \textbf{pass@5} \\
\midrule
Python $\rightarrow$ Java   & 89.6 & 90.2 & 88.4 & 91.5 & 90.8 & $90.1 \pm 1.1$ & 95.1 \\
Python $\rightarrow$ C      & 82.3 & 83.5 & 81.7 & 84.1 & 82.9 & $82.9 \pm 0.9$ & 88.4 \\
Python $\rightarrow$ C++    & 85.4 & 86.2 & 84.8 & 87.1 & 85.9 & $85.9 \pm 0.8$ & 91.5 \\
Python $\rightarrow$ Go     & 79.3 & 80.1 & 78.7 & 81.2 & 79.8 & $79.8 \pm 0.9$ & 85.4 \\
\midrule
\textbf{Average}            & 84.2 & 85.0 & 83.4 & 86.0 & 84.9 & $84.7 \pm 1.0$ & 90.1 \\
\bottomrule
\end{tabular}%
}
\end{table}

\pa{Result.} Table~\ref{tab:rq4_stability} summarizes the results across five independent runs of \tool{} on the EvalPlus dataset. The low standard deviation ($\leq 1.2\%$) across all target languages confirms that the pipeline produces stable and consistent results despite using a non-deterministic temperature. The pass@5 scores are consistently higher than single-run CA, reflecting that independent re-execution reliably recovers from occasional translation failures. Specifically, for Python$\rightarrow$Java, \tool{} achieves a mean CA of \TODO\% with a standard deviation of \TODO\%, and a pass@5 of \TODO\%. These results demonstrate that the non-determinism introduced by temperature = 0.8 does not undermine the reliability of \tool{}, and that the pipeline converges to stable performance across independent executions.
}
